A Call to Reflect on Evaluation Practices for Age Estimation: Comparative Analysis of the State-of-the-Art and a Unified Benchmark

Comparing different age estimation methods poses a challenge due to the unreliability of published results stemming from inconsistencies in the benchmarking process. Previous studies have reported continuous performance improvements over the past decade using specialized methods; however, our findings challenge these claims. This paper identifies two trivial, yet persistent issues with the currently used evaluation protocol and describes how to resolve them. We offer an extensive comparative analysis for state-of-the-art facial age estimation methods. Surprisingly, we find that the performance differences between the methods are negligible compared to the effect of other factors, such as facial alignment, facial coverage, image resolution, model architecture, or the amount of data used for pretraining. We use the gained insights to propose using FaRL as the backbone model and demonstrate its effectiveness on all public datasets. We make the source code and exact data splits public on GitHub.

==> X_rebuttal.tex <==
\clearpage
\twocolumn
\pagenumbering{gobble}
\thispagestyle{empty}
\appendix
\setlength{\parskip}{-6pt}
\maketitlerebuttal

\noindent We appreciate the valuable feedback from reviewers  {\bf\color{review1}\hbox{R1: 57oT}}, {\bf\color{review2}R2: oZzE}, and 
{\bf\color{review3}R3: vzMF}. In response to their insightful comments, we will incorporate the feedback.

\paragraph{Contributions}\hspace{-0.5em}
\hspace{-0.5em}\revone correctly points out that the proposed fix is trivial. However, the addressed issue is pervasive. We firmly believe that despite the simplicity of the proposed solution the primary message of our paper is important.

\paragraph{Task Analysis}\hspace{-0.5em}\revone inquires about the uncertainty of the task. The irreducible Bayes error is contingent on the specific formulation. When estimating the \textit{real age} from an observation $x_i$, the label $y_i$ is a realization of the distribution $p(y\,|\,x)$, a random variable. The observation $x_i$ does not contain all the necessary information about the person's genetics, lifestyle, etc., and the Bayes error is non-zero. Interestingly, when estimating the \textit{apparent age}, the Bayes error can be 0. Specifically, when the label is defined as $y_i = \mathbb{E}_{\hat y_i \sim p(y\,|\,x)}[{\hat y_i}]$, which is \textit{not} a random variable. Apparent age is by definition the expected annotation provided by observers. Therefore the observation $x_i$ must necessarily contain all the information used to generate the label. The process of dataset collection provides further insight. For AgeDB, AFAD, and CACD2000, the age label is defined as the \textit{year when the photo was taken} minus the \textit{year of birth}. Two individuals born on December 31st and January 1st would thus have different age labels, even though they were born just a day apart. The \textit{year taken} and the \textit{year born} can also be noisy. For instance, AFAD collects data from a social network with a minimum age requirement of 15, without verifying the actual age of the users. CLAP2016, FG-NET, and MORPH use the legal age as the age label. Still, uncertainty arises from the discrete nature of the label. For UTKFace, the labels are estimated by DEX \cite{DEX}, and manually verified. Therefore, DEX should attain zero error on UTKFace.

\paragraph{Hyperparameters \& Preprocessing}\hspace{-0.5em}\revtwo questions the choice of hyperparameters and preprocessing for different loss functions. We want to clarify that we do \textit{not} tune the hyperparameters of the methods \cite{OR-CNN, DLDL, DLDL-V2, SoftLabels, MeanVariance, Unimodal} on the validation set. We apply them in the original configurations. \revtwo is correct that we do not search for optimal training hyperparameters or preprocessing; we maintain a consistent setting across all experiments. We argue that if any of the loss functions is a significant improvement over the baseline, we should observe a performance improvement across a broad range of hyperparameters and preprocessing pipelines. Instead, we find that the specialized loss functions only improve performance when the models are initialized randomly. This is consistent across all datasets.

\paragraph{Literature Review}\hspace{-0.5em}\revone asks about the percentage of papers that adopt a generic architecture by changing its last layer or the loss function. Our estimates, based on the surveyed literature (see Appendix), indicate that approximately $70\%$ of the papers that attempt to improve age estimation follow this approach. Only a minority of these papers adequately ablate the impact of the proposed modifications. Most of the remaining papers suggest modifications to the training procedure, backbone, or aspects of the data pipeline.

\paragraph{Best Practices}\hspace{-0.5em}\revtwo raises questions about our choices in pre-training and backbone selection. We observe that from all the compared factors, the amount of data used for pre-training has the largest impact on model performance. Consequently, we attempt to utilize as much data for pre-training as possible. The FaRL \cite{FaRL} backbone utilizes a substantial set of 20 million facial images. It is worth noting that these images are annotated not by age but by text description. Our decision to use FaRL is driven solely by the extensive amount of pre-training data it incorporates, rather than specific characteristics of the backbone. Different image encoders could be trained in the same manner. However, due to the costs associated with training such models, we have chosen to reuse the FaRL ViT-B-16 backbone.


%\paragraph{Classification, Regression, or Ordinal Regression?}\hspace{-0.5em}\revone Show experimentally results between classification, regression and ordinal regression

\paragraph{Terminology}\hspace{-0.5em}\revthree correctly highlighted that the term \textit{subject-exclusive} is not standard in the literature. Following the recommendation, we have opted to use the term \textit{identity-disjoint}. We will explicitly mention in the paper that various terms can be found in the literature for the same concept.

\paragraph{Ethical Concerns}\hspace{-0.5em}\revone questions broader implications and ethical concerns of our work. We aim to facilitate tangible improvements in age estimation and collaboration among researchers by standardizing the setup. The ethical considerations of our work are therefore closely tied to the broader concerns surrounding age estimation technology. Similar to other biometric techniques, age estimation can be applied in forensic analysis, child protection, surveillance, and various other contexts. These technologies have the potential to aid in identifying individuals and monitoring their activities, leading to the apprehension of criminals. However, this also raises concerns about potential discrimination and government surveillance of citizens. Ongoing discussions, particularly in the EU legislative framework, focus on establishing regulations for the ethical deployment of age estimation methods in different contexts. One of the major concerns revolves around the accuracy and reliability of these methods. Age estimation results may not always be precise. While the private sector offers certificates to validate the reliability of these algorithms, ethical dilemmas persist.
